How Much Has Embodied AI Progressed? A Meta-Analysis on Robot Manipulation Benchmarks vs. VLA, WAM, and LLM Agents

Robot manipulation policies, from vision-language-action models (VLAs) and world-action models (WAMs) to, most recently, large language model (LLM) agents, now improve within months. However, each benchmark separates them only over a narrow range: older benchmarks saturate, while on newer ones most policies score in the single digits, so policies evaluated on different benchmarks cannot be compared and the pace of progress cannot be measured. We place policy capabilities and task difficulties from different benchmarks on one Elo scale, linking the benchmarks through the policies they share, as test linking does for exams in educational measurement; on this scale, a policy's odds of success on a task are the ratio of its capability to the task's difficulty. Applied to 44 policies released between December 2022 and October 2026 on LIBERO, SimplerEnv, RoboTwin 2.0 and RoboDojo (212 test cases, 395,092 trials), the scale predicts a policy's results on a benchmark hidden from the fit with an error of 6.8 points in mean score, against 11.9 for the per-task average. On this unified scale, today's best policy is about 18 times as capable as RT-1. On average, policy capability doubled every 8.5 months, and since June 2026 the best policy has improved about ten times as fast as before. Meanwhile, the difficulty of new benchmarks grew about 8.5-fold a year (95% CI: 2-36): the median task of today's hardest benchmark, RoboDojo, is about 1,200 times as difficult as LIBERO's. Benchmarks that were hard at release saturated 7 to 21 months later, and every benchmark except RoboDojo is already saturated. If the pace since June 2026 holds, the best policy will saturate RoboDojo around September 2027, and the tasks that remain hard, open-ended tasks in randomized scenes, are where the next benchmark should build.

==> sections/tab_linking.tex <==
RoboDojo & 19 & 0.228 & 0.281 & 3.9 & 4.4 & 9.8 & 85\% \\
RoboTwin & 14 & 0.511 & 0.598 & 9.6 & 8.0 & 18.5 & 84\% \\
LIBERO & 19 & 0.249 & 0.248 & 6.4 & 5.5 & 7.5 & 71\% \\
SimplerEnv & 9 & 0.585 & 0.613 & 9.4 & 10.1 & 15.5 & 72\% \\


==> sections/tab_policies.tex <==
1 & WALL-OSS-1.0-lite~\citep{xsquare2026wallosslite} & 2026-10 & 2078 & 2019--2151 & D \\
2 & PrismWAM$^{*}$~\citep{xin2026prismwam} & 2026-10 & 2056 & 2023--2098 & TD \\
3 & VPP2~\citep{guo2026vpp2} & 2026-10 & 2042 & 1994--2100 & D \\
4 & PatchWAM~\citep{wang2026patchwam} & 2026-09 & 1990 & 1958--2034 & T \\
5 & InternW0-$\Delta$~\citep{miao2026internw0} & 2026-09 & 1970 & 1931--2016 & D \\
6 & GPT-6-Astra$^{\ddagger}$~\citep{openai2026gpt6astra} & 2026-09 & 1953 & 1857--2053 & D \\
7 & PrismWAM~\citep{xin2026prismwam} & 2026-10 & 1928 & 1902--1964 & TD \\
8 & EWAM~\citep{wang2026ewam} & 2026-09 & 1909 & 1882--1942 & TD \\
9 & Xiaomi-R1~\citep{xiaomi2026r1} & 2026-07 & 1871 & 1837--1912 & D \\
10 & OpenDM0.5~\citep{dexmal2026dm05} & 2026-07 & 1864 & 1815--1917 & LD \\
11 & GigaBrain-0.7~\citep{gigabrain2026gigabrain07} & 2026-08 & 1845 & 1813--1881 & T \\
12 & G0.5~\citep{galaxea2026g05} & 2026-06 & 1821 & 1783--1865 & LTD \\
13 & LingBot-VA~\citep{li2026lingbotva} & 2026-01 & 1801 & 1737--1893 & L \\
14 & hy-vla~\citep{zhang2026hyvla} & 2026-06 & 1763 & 1729--1803 & D \\
15 & $\pi_{0.5}$~\citep{pi2025pi05} & 2025-04 & 1762 & 1741--1790 & LTD \\
16 & InternVLA-A1.5~\citep{ma2026internvlaa15} & 2026-07 & 1759 & 1726--1794 & LD \\
17 & InternVLA-M1~\citep{chen2025internvlam1} & 2025-10 & 1737 & 1685--1812 & LS \\
18 & MolmoAct2~\citep{fang2026molmoact2} & 2026-05 & 1730 & 1683--1783 & LD \\
19 & Xiaomi-R0~\citep{cai2026xiaomir0} & 2026-02 & 1713 & 1688--1744 & LSTD \\
20 & X-VLA~\citep{zheng2025xvla} & 2025-10 & 1707 & 1661--1752 & LSTD \\
21 & VLA-JEPA~\citep{sun2026vlajepa} & 2026-02 & 1700 & 1658--1747 & LS \\
22 & CogACT~\citep{li2024cogact} & 2024-11 & 1698 & 1636--1772 & S \\
23 & ABot-M0~\citep{yang2026abotm0} & 2026-02 & 1659 & 1626--1697 & LTD \\
24 & UniVLA~\citep{bu2025univla} & 2025-05 & 1632 & 1582--1682 & LS \\
25 & SpatialVLA~\citep{qu2025spatialvla} & 2025-01 & 1591 & 1480--1687 & S \\
26 & RT-1~\citep{brohan2022rt1} & 2022-12 & 1578 & 1528--1646 & S \\
27 & GR00T N1.7~\citep{nvidia2025gr00tn1} & 2026-03 & 1570 & 1532--1604 & LSD \\
28 & GR00T N1.6~\citep{nvidia2025gr00tn1} & 2025-12 & 1566 & 1453--1678 & S \\
29 & MolmoAct~\citep{lee2025molmoact} & 2025-08 & 1535 & 1494--1579 & LS \\
30 & FastWAM~\citep{yuan2026fastwam} & 2026-03 & 1524 & 1453--1573 & LTD \\
31 & GR00T N1.5~\citep{nvidia2025gr00tn1} & 2025-05 & 1522 & 1480--1556 & LS \\
32 & $\pi_0$-FAST~\citep{pertsch2025fast} & 2025-01 & 1498 & 1453--1539 & L \\
33 & DeepSeek-Flash$^{\ddagger}$~\citep{deepseek2026v41flash} & 2026-09 & 1490 & 1356--1602 & D \\
34 & starVLA~\citep{ye2026starvla} & 2026-04 & 1464 & 1426--1500 & TD \\
35 & $\pi_0$~\citep{black2024pi0} & 2024-10 & 1460 & 1440--1483 & LTD \\
36 & RDT-1B~\citep{liu2024rdt} & 2024-10 & 1373 & 1347--1403 & TD \\
37 & SmolVLA~\citep{shukor2025smolvla} & 2025-06 & 1367 & 1333--1401 & LTD \\
38 & OpenVLA-OFT~\citep{kim2025openvlaoft} & 2025-02 & 1366 & 1315--1408 & LD \\
39 & GPT-5.5$^{\ddagger}$~\citep{openai2026gpt55} & 2026-04 & 1338 & 1143--1477 & D \\
40 & RT-1-X~\citep{oxe2023rtx} & 2023-10 & 1327 & 1251--1407 & S \\
41 & OpenVLA~\citep{kim2024openvla} & 2024-06 & 1302 & 1257--1341 & LS \\
42 & ACT~\citep{zhao2023act} & 2023-04 & 1268 & 1211--1311 & TD \\
43 & Octo~\citep{octo2024octo} & 2024-05 & 1242 & 1149--1314 & S \\
44 & DP~\citep{chi2023diffusion} & 2023-03 & 1188 & 1058--1246 & T \\

